HiCM$^2$: Hierarchical Compact Memory Modeling for Dense Video Captioning

With the growing demand for solutions to real-world video challenges, interest in dense video captioning (DVC) has been on the rise. DVC involves the automatic captioning and localization of untrimmed videos. Several studies highlight the challenges of DVC and introduce improved methods utilizing prior knowledge, such as pre-training and external memory. In this research, we propose a model that leverages the prior knowledge of human-oriented hierarchical compact memory inspired by human memory hierarchy and cognition. To mimic human-like memory recall, we construct a hierarchical memory and a hierarchical memory reading module. We build an efficient hierarchical compact memory by employing clustering of memory events and summarization using large language models. Comparative experiments demonstrate that this hierarchical memory recall process improves the performance of DVC by achieving state-of-the-art performance on YouCook2 and ViTT datasets.

==> setup/macros.tex <==
% Macros - Jia-Bin Huang (jbhuang@vt.edu)

\renewcommand{\baselinestretch}{0.96}       % for squeezing the draft into the page limit, do not use

% =========================================
% Useful macros
% =========================================

% Latin abbreviations
\def\etal{et~al.\_}			  % and others, and co-workers
\def\Eg{E.g.,~}               % for example
\def\eg{e.g.,~}               % for example
\def\ie{i.e.,~}               % that is, in other words
\def\etc{etc}                 % and other things, and so forth
\def\cf{cf.~}                 % compare
\def\viz{viz.~}               % namely, precisely
\def\vs{vs.~}                 % against

\def\naive{na{\"i}ve\xspace}
\def\Naive{Na{\"i}ve\xspace}
\def\Naively{Na{\"i}vely\xspace}

% Math related
\DeclareMathOperator*{\argmin}{\arg\!\min} 
\DeclareMathOperator*{\argmax}{\arg\!\max}

% Consistent margin adjustment for paragraphs, figures, and sections
\newlength\paramargin
\newlength\figmargin

\newlength\secmargin
\newlength\figcapmargin
\newlength\tabcapmargin

\setlength{\secmargin}{-2.0mm}
\setlength{\paramargin}{-2.0mm}
\setlength{\figmargin}{0.0mm}
\setlength{\tabcapmargin}{-3.0mm}

\setlength{\figcapmargin}{-4.0mm}

\setlength{\fboxsep}{0pt}

\newcommand{\red}{\textcolor{red}}
\newcommand{\blue}{\textcolor{blue}}

% minipage
\newcommand{\mpage}[2]
{
\begin{minipage}{#1\linewidth}\centering
#2
\end{minipage}
}

\newcommand{\mfigure}[2]
{
\includegraphics[width=#1\linewidth]{#2}
}

\newcommand{\heading}[1]
{
\vspace{1mm}\noindent\textbf{#1}
}


\newcommand{\topic}[1]
{
\paramargin\noindent \textbf{#1}
}

\newcommand{\figcaption}[2]
{
\caption{
\textbf{#1.}  % Figure caption title
#2            % Caption
}
}

% References for figures, tables, equations, and sections
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}} 
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\appenref}[1]{Appendix \S ~\ref{appen:#1}}
\newcommand{\eqnref}[1]{\eqref{eq:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\prgref}[1]{Program~\ref{#1}}
\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\clmref}[1]{Claim~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\ptyref}[1]{Property~\ref{#1}}

% Comments
\long\def\ignorethis#1{}
\newcommand {\jw}[1]{{\color{cyan}\textbf{Jinwoo: }#1}\normalfont}
\newcommand {\st}[1]{{\color{red}\textbf{Seong Tae: }#1}\normalfont}
\newcommand {\Minkuk}[1]{{\color{magenta}\textbf{Minkuk: }#1}\normalfont}
\newcommand {\Hyeonbae}[1]{{\color{green}\textbf{Hyeonbae: }#1}\normalfont}

\newcommand {\todo}{{\textbf{\color{red}[TO-DO]\_}}}
\def\newtext#1{\textcolor{blue}{#1}}
\def\modtext#1{\textcolor{red}{#1}}
\newcommand{\note}[1]{{\it\color{blue} #1}}

\newcommand{\tb}[1]{\textbf{#1}}
\newcommand{\mb}[1]{\mathbf{#1}}

\newcommand{\jbox}[2]{
  \fbox{%
  	\begin{minipage}{#1}%
  		\hfill\vspace{#2}%
  	\end{minipage}%
  }}

\newcommand{\jblock}[2]{%
	\begin{minipage}[t]{#1}\vspace{0cm}\centering%
	#2%
	\end{minipage}%
}

% subfigures with automatic width
\newbox\jsavebox%
\newcommand{\jsubfig}[2]{%
	\sbox\jsavebox{#1}%
	\parbox[t]{\wd\jsavebox}{\centering\usebox\jsavebox\\#2}%
	}


\newcommand{\best}[1]{{\textbf{#1}}}
\newcommand{\second}[1]{{\underline{#1}}}
\newcommand{\appsection}[2]{
  \hspace{2cm}$\bullet$\hspace{0.2cm}#1 $\rightarrow$ \S\ref{appen:#2}
}


==> table/07_scalability_abl.tex <==

\begin{table}
% \begin{table}[]
\centering
\begin{tabular}{c|cccc}
\toprule
Memory &\multirow{2}{*}{ CIDEr} & \multirow{2}{*}{METEOR }& \multirow{2}{*}{SODA\_c}&\multirow{2}{*}{ F1} \\
Data & &  & & \\
\midrule
No Mem         & 66.29 & 12.41 & 9.87  & 31.08 \\
Target         & \textbf{71.84} & \textbf{12.80} & \textbf{10.73} & \textbf{32.51} \\
In-domain      &       &       &       &       \\
In\&Out-domain & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ 
\bottomrule
\end{tabular}
\caption{The effect of Memory Bank Scale.}
\label{tab:scalability_abl}
\end{table}
